On the Approximation Properties of Random ReLU Features

We study the approximation properties of random ReLU features through their reproducing kernel Hilbert space (RKHS). We first prove a universality theorem for the RKHS induced by random features whose feature maps are of the form of nodes in neural networks. The universality result implies that the random ReLU features method is a universally consistent learning algorithm. We prove that despite the universality of the RKHS induced by the random ReLU features, composition of functions in it generates substantially more complicated functions that are harder to approximate than those functions simply in the RKHS. We also prove that such composite functions can be efficiently approximated by multi-layer ReLU networks with bounded weights. This depth separation result shows that the random ReLU features models suffer from the same weakness as that of shallow models. We show in experiments that the performance of random ReLU features is comparable to that of random Fourier features and, in general, has a lower computational cost. We also demonstrate that when the target function is the composite function as described in the depth separation theorem, 3-layer neural networks indeed outperform both random ReLU features and 2-layer neural networks.

==> pf_sep_barron.tex <==
To prove Proposition~\ref{prop:separation}, we only need to check the
Remark 4 of \cite{Eldan2016}, which states that not only is the width of
the 3-layer network of size $ \mathrm{poly}(d) $, but also all the parameters are
$ \mathrm{poly}(d) $. If the claim is true, the following argument completes
the proof. The 3-layer network $ g $ is the composite of 2 2-layer
networks, and each of the 2-layer network belongs to $ \Lambda_{\mathrm{poly}(d)} $
by the definition of ReLU feature class. And since $ g $ cannot be approximated
by any 2-layer networks with fewer than $ c\exp(cd) $ nodes, it cannot be
approximated by any function in $ \Lambda_{D} $ with $ D\le c\exp(cd) $.
Otherwise it will contradict the fact that any function in $ \Lambda_D $
can be approximated by a 2-layer ReLU network with $ O(D^2) $ nodes. Now
we check the remark. For convenience, we will directly use the notation in
\cite{Eldan2016} without defining them.
\begin{proposition*}[\ref{prop:separation}]
  There exists universal constants $ c,C $ such that for any $ d>C $,
  there exists a probability measure $ \mu $ supported on a compact set of
  $ \mathbb{R}^d $, and two functions $ f:\mathbb{R}^d\to\mathbb{R} $ and
  $ g:\mathbb{R}\to\mathbb{R} $
  with the following properties:
  \begin{enumerate}
    \item the functions $ f $ and $ g $ belong to $ \Lambda_{Cd^{6.25}} $ and
    $ \Lambda_{Cd^{4.5}} $ respectively,
    \item and every function $ h $ in $ \Lambda_{D} $ with $ D\le ce^{cd} $
    satisfies
    \begin{equation*}
      \Vert h-f\circ g\Vert_{L^2(\mu)} \ge c\,.
    \end{equation*}
  \end{enumerate}
\end{proposition*}
\begin{proof}
The 3-layer ReLU network is the composition of 2 2-layer ReLU networks, $ \tilde{\ell} $
and $ \tilde{s} $. $ \tilde{\ell} $ approximates the function
$ \ell:\mathbb{R}^d\to\mathbb{R} $, and $ \tilde{s} $ approximates
$ s:\mathbb{R}\to\mathbb{R} $, as defined in the proof of Lemma~18 of Eldan and
Shamir's work.
By Lemma~19 in Appendix~A of Eldan and Shamir's work, when the activation node
is ReLU, $ c_\sigma \le 4 $. And $ \tilde{\ell} $ has the form
\[
  \sum_{i=1}^d(a+\sum_{j=1}^w\alpha_i\sigma(\mathbf{e}_i\cdot \mathbf{x}-\beta_i))\,.
\]
Since $ \ell $ is $ 2R $-Lipschitz, when
\[
  \sup_{\mathbf{x}\le\mathbb{R}^d}\left\vert\tilde{\ell}(\mathbf{x})
  -\ell(\mathbf{x})\right\vert \le \frac{\sqrt{r}\delta}{N}\,,
\]
we have $ a = R^2 $, $ \vert\alpha_i\vert \le 2R $,
$ \vert\beta_i\vert \le 2R $ and $ w \le \frac{8dR^2N}{\sqrt{r}\delta} $.
Since $ s $ is $ \frac{N}{2\sqrt{r}} $-Lipschitz and supported on the interval
$ [-R^2,R^2] $, to get
\[
  \sup_{x\in\mathbb{R}}\left\vert\tilde{s}(x)-s(x)\right\vert < \delta/2\,,
\]
we have
\[
  \tilde{s}(x) =  a' + \sum_{i=1}^{w'}\alpha'_i\sigma(x-\beta'_i)\,,
\]
where $ a' = 0 $, $ \vert\alpha'_i\vert \le \frac{N}{\sqrt{r}} $,
$ \vert\beta'_i\vert \le 2R^2 $, and $ w' \le \frac{4R^2N}{\sqrt{r}\delta} $.
Together with the fact that $ N = C(\alpha d)^{3/2} $, $ r = \alpha\sqrt{d} $,
and $ R = 2\alpha \sqrt{d} $, we have
$ \tilde{\ell} \in \Lambda_{C_{\alpha,\delta}d^{6.25}} $
and $ \tilde{s}\in\Lambda_{C_{\alpha,\delta}d^{4.5}} $. For sufficiently small
$ \delta $ and large $ \alpha $, we have $ \tilde{s}\circ\tilde{\ell} $ is far
from any 2-layer ReLU network with number of nodes $ D\le ce^{cd} $ by a constant
under $ L^2(\varphi^2) $ distance. Note that $ \varphi^2 $ is a probability
distribution over $ \mathbb{R}^d $, but the composite function $ \tilde{s}\circ\tilde{\ell} $
is only supported over the annulus $ \alpha\sqrt{d}\le\Vert x\Vert\le 2\alpha\sqrt{d} $.
And hence, we can set $ \mathcal{X} $ to be the annulus. And define a
probability measure $ \mu = \varphi^2/\varphi^2(\mathcal{X}) $. Then $ \tilde{s}\circ\tilde{\ell} $
is still far from any 2-layer ReLU network with number of nodes $ D\le ce^{cd} $ by a constant
under $ L^2(\mu) $ distance. By Theorem~\ref{thm:main}, any function in
$ \Lambda_D(\mathcal{X}) $ can be approximated by 2-layer ReLU networks
with $ D^2(4\alpha^2d+1) $ nodes. Therefore we conclude that all functions in
$ \Lambda_D $ with $ D\le ce^{cd} $ are away from $ \tilde{s}\circ\tilde{\ell} $
by constant $ L^2(\mu) $ distance.
\end{proof}


